Counterfactual Depth from a Single RGB Image

We describe a method that predicts, from a single RGB image, a depth map that describes the scene when a masked object is removed - we call this "counterfactual depth" that models hidden scene geometry together with the observations. Our method works for the same reason that scene completion works: the spatial structure of objects is simple. But we offer a much higher resolution representation of space than current scene completion methods, as we operate at pixel-level precision and do not rely on a voxel representation. Furthermore, we do not require RGBD inputs. Our method uses a standard encoder-decoder architecture, and with a decoder modified to accept an object mask. We describe a small evaluation dataset that we have collected, which allows inference about what factors affect reconstruction most strongly. Using this dataset, we show that our depth predictions for masked objects are better than other baselines.

==> table-masked.tex <==
\begin{table}
\begin{center}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{|c||c|c||c|c|c|}
\hline
Method & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
\hline
Do nothing
    & 0.492     & 0.216     & 48.2      & 86.1      & 99.6 \\
Poisson \cite{perez2003poisson}
    & 0.366     & 0.157     & 70.4      & 96.9      & \bf 100.0 \\
Inpaint \cite{iizuka2017globally}
    & 0.506     & 0.232     & 57.2      & 95.2      & \bf 100.0 \\
DepthComp~\cite{atapour2017depthcomp}
    & 0.467     & 0.191     & 62.8      & 93.3      & 99.9 \\
Auto-encoder
    & 0.344     & 0.141     & 78.1      & 98.4      & \bf 100.0 \\
Ours
    & \bf 0.310 & \bf 0.132 & \bf 81.7  & \bf 99.5  & \bf 100.0 \\
\hline
\end{tabular}}
\end{center}
%\vspace{-0.5mm}
\caption{Depth prediction~(object removed) performance comparison on our collected evaluation dataset. Here we evaluate {\bf masked image pixels only.} We compare with the five natural baselines, our approach without the surface normal loss and our approach without mask drop out.  Note the surface normal loss and mask drop out both help our method significantly.  Our method
outperforms baselines by a substantial margin.  Poisson and do nothing in fact perform rather worse than our method {\em on the pixels that matter}.
} %Metric from left to right: root mean square, absolute relative difference, $\delta <1.25$, $\delta <1.25^2$, and $\delta <1.25^3$.} %Note in left columns lower is better, while higher is better in right columns.}
\label{table:depthin}
\end{table}


==> table-nonmasked.tex <==
\begin{table}
\begin{center}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{|c||c|c||c|c|c|}
\hline
Method & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
\hline
Do nothing                      & 0.462 & 0.227 & 64.9 & 88.8 &  99.8\\
Poisson \cite{perez2003poisson} & 0.453 & 0.222 & 66.6 & 89.6 & 99.8\\
Inpaint \cite{iizuka2017globally}              & 0.516 & 0.245 & 63.0 & 87.7 &  99.8\\
DepthComp~\cite{atapour2017depthcomp}               & 0.461 & 0.226 & 65.6 & 89.3 & \textbf{99.9}\\
Auto-encoder                 & 0.430 & 0.210 & 69.4 & 91.2 & \textbf{99.9}\\
Ours                            & \bf 0.426 & \bf 0.199 & \bf 70.4 & \bf 93.0 & 99.8\\
\hline
\end{tabular}}
\end{center}
%\vspace{-0.5mm}
\caption{Depth prediction~(object removed) performance comparison on our collected evaluation dataset. Here we evaluate {\bf {\color{red} non-masked pixels}}  
We compare with the five natural baselines, our approach without the surface normal loss and our approach without mask drop out.  Note the surface normal loss and mask drop out both help our method significantly. Our method
outperforms baselines by a substantial margin.  While both Poisson and do nothing look quite good, this is an artifact of the measurement.
} %Metric from left to right: root mean square, absolute relative difference, $\delta <1.25$, $\delta <1.25^2$, and $\delta <1.25^3$.} %Note in left columns lower is better, while higher is better in right columns.}
\label{table:depthwhole}
\end{table}

==> table-sup-ai2thor.tex <==
\begin{table*}[!h]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
\hline
    & \multicolumn{6}{c||}{All Pixels}
    & \multicolumn{6}{c||}{Interior}
    & \multicolumn{6}{c|}{Exterior} \\
\cline{2-19}
Method
    & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
    & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
    & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
\hline
& \multicolumn{18}{c|}{Input depth map: Laina \etal}\\
\hline
Do nothing
    &     .875 &    .659 &    .289 &    49.2 &    77.6 &    91.8
    &    1.094 &    .867 &    .267 &    40.7 &    71.5 &    88.6
    &     .867 &    .651 &    .288 &    49.8 &    78.2 &    92.0\\
Poisson% \cite{perez2003poisson}
    &     .875 &    .658 &    .289 &    49.4 &    77.7 &    91.7
    &    1.088 &    .846 &    .259 &    43.9 &    72.7 &    89.5
    &*&*&*&*&*&*\\
DepthComp%~\cite{atapour2017depthcomp}
    &     .876 &    .659 &    .289 &    49.2 &    77.6 &    91.8
    &    1.094 &    .867 &    .267 &    40.6 &    71.5 &    88.6
    &*&*&*&*&*&*\\
Inpaint% \cite{iizuka2017globally}
    &     .893 &    .672 &    .294 &    48.3 &    76.2 &    91.1
    &    1.050 &    .809 &    .246 &    47.3 &    73.1 &    90.8
    &     .888 &    .668 &    .294 &    48.6 &    76.5 &    91.1\\
Auto-encoder
    &     .898 &    .672 &    .284 &    47.8 &    76.5 &    91.2
    &    0.999 &    .770 &    .232 &    48.5 &    78.3 &    93.9
    &     .896 &    .670 &    .285 &    47.9 &    76.6 &    91.1\\
\hline
& \multicolumn{18}{c|}{Input depth map: Ours with empty object mask}\\
\hline
Do nothing
    &     .548 &    .364 &    .158 &    75.6 &    92.5 &    98.0
    &    0.667 &    .498 &    .158 &    68.6 &    92.3 &    98.8
    &     .539 &    .357 &    .156 &    76.4 &    93.0 &\bf 98.2\\
Poisson% \cite{perez2003poisson}
    &     .548 &    .363 &    .158 &    75.9 &    92.6 &    97.9
    &    0.691 &    .492 &    .156 &    72.2 &    92.6 &    97.3
    &*&*&*&*&*&*\\
DepthComp%~\cite{atapour2017depthcomp}
    &     .546 &    .361 &    .158 &    76.0 &    92.7 &    98.1
    &    0.684 &    .490 &    .157 &    71.6 &    92.6 &    97.9
    &*&*&*&*&*&*\\
Inpaint% \cite{iizuka2017globally}
    &     .582 &    .386 &    .165 &    73.8 &    91.3 &    97.6
    &    0.665 &    .479 &    .152 &    73.9 &    92.8 &    98.5
    &     .577 &    .381 &    .164 &    74.2 &    91.5 &    97.8\\
Auto-encoder
    &     .578 &    .390 &    .163 &    73.6 &    91.6 &    98.0
    &    0.602 &    .441 &    .139 &    77.1 &\bf 95.3 &\bf 99.7
    &     .577 &    .388 &    .163 &    73.7 &    91.7 &    98.0\\
\hline
Ours
    & \bf .542 &\bf .359 &\bf .157 &\bf 76.3 &\bf 92.9 &\bf 98.2
    &\bf 0.592 &\bf .423 &\bf .138 &\bf 78.9 &    95.3 &    99.4
    & \bf .539 &\bf .356 &\bf .156 &\bf 76.4 &\bf 93.0 &    98.2\\
\hline
% Ours w/o mask
%     &     .442 &    .301 &    .163 &    77.3 &\bf 95.1 &    98.4
%     & \bf .384 &    .269 &    .120 &    86.2 &\bf 98.3 &    99.8
%     &     .442 &    .301 &    .164 &    77.3 &\bf 95.1 &    98.4\\
% Ours w/o norm
%     &     .522 &    .358 &    .192 &    72.6 &    91.6 &    96.9
%     &     .470 &    .330 &    .149 &    80.4 &    95.9 &    98.9
%     &     .522 &    .357 &    .192 &    72.7 &    91.6 &    96.9\\
% \hline
\end{tabular}
}%resizebox
\end{center}
\vspace{-1mm}
\caption{Depth prediction~(with object removed) performance compared with other baselines on AI2-THOR test samples. We evaluate average pixel performance on: left: all image pixels, middle: pixels inside the object mask~(interior), and right: pixels outside the object mask~(exterior). ``*'' in exterior columns means that the method does not produce pixels in this region. We also compare with two different input depth maps for the baselines, Laina~\etal, and ours with empty object mask (also shown as Table 2 on the main paper). In this case, using ours as the input depth map results in better performance for other baselines.% Autoencoder performs slightly better than ours in some metrics but it trashes at pixels outside the object mask.
%Poisson and DepthComp only produce pixels within mask; that's why we report * in exterior columns where the values are equal to Do nothing. Our method outperforms baselines.
%The last block is only for an ablation study of our network. We study the effect (or lack) of mask dropout (ours w/o mask) and normal loss (ours w/o normal). They make our network (ours) more reliable on both interior and exterior regions. 
}
% To better compare with these we make a special method to Autoencoder (C\&P AE) and ours (C\&P Ours) by copy and paste the exterior from the initial depth. Thus these C\&P methods have the same exterior, hence we clearly see the result of interior pixels.
%\vspace{-1mm}
%Metric from left to right: root mean square, absolute relative difference, $\delta <1.25$, $\delta <1.25^2$, and $\delta <1.25^3$.} %Note in left columns lower is better, while higher is better in right columns.}
\label{table:supai2thorsel}
\end{table*}







% \begin{table*}[!h]
% \begin{center}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
% \hline
%     & \multicolumn{6}{c||}{All Pixels}
%     & \multicolumn{6}{c||}{Interior}
%     & \multicolumn{6}{c|}{Exterior} \\
% \cline{2-19}
% Method
%     & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
% \hline
% & \multicolumn{18}{c|}{Initial depth predictor: Laina}\\
% \hline
% Do nothing
%     &     .743 &    .556 &    .306 &    50.9 &    79.7 &    92.5
%     &     .727 &    .519 &    .216 &    57.6 &    85.2 &    95.9
%     &     .743 &    .556 &    .309 &    50.9 &    79.6 &    92.4\\
% Poisson% \cite{perez2003poisson}
%     &     .743 &    .555 &    .306 &    51.0 &    79.7 &    92.4
%     &     .734 &    .520 &    .217 &    57.9 &    84.5 &    94.7
%     &*&*&*&*&*&*\\
% DepthComp%~\cite{atapour2017depthcomp}
%     &     .743 &    .556 &    .307 &    50.9 &    79.7 &    92.5
%     &     .727 &    .519 &    .217 &    57.5 &    85.2 &    95.9
%     &*&*&*&*&*&*\\
% Inpaint% \cite{iizuka2017globally}
%     &     .758 &    .565 &    .312 &    50.5 &    79.0 &    91.5
%     &     .733 &    .521 &    .222 &    58.2 &    84.2 &    95.3
%     &     .758 &    .566 &    .314 &    50.5 &    78.9 &    91.4\\
% Auto-encoder
%     &     .750 &    .556 &    .293 &    50.0 &    79.2 &    93.0
%     &     .700 &    .506 &    .219 &    58.1 &    85.4 &    96.8
%     &     .750 &    .555 &    .294 &    50.0 &    79.2 &    93.0\\
% \hline
% & \multicolumn{18}{c|}{Initial depth predictor: Ours w/o object mask}\\
% \hline
% Do nothing
%     &     .436 &    .290 &    .155 &    79.5 &    94.7 &    98.5
%     &     .414 &    .280 &    .118 &    85.9 &    97.5 &    99.7
%     & \bf .434 &\bf .289 &    .155 &\bf 79.6 &\bf 94.8 &\bf 98.6\\
% \hline
% Poisson% \cite{perez2003poisson}
%     &     .438 &    .291 &    .156 &    79.2 &    94.5 &    98.4
%     &     .455 &    .300 &    .133 &    83.7 &    95.1 &    97.5
%     %& \bf .434 &\bf .289 &    .155 &\bf 79.6 &    94.8 &\bf 98.6\\
%     &*&*&*&*&*&*\\
% DepthComp%~\cite{atapour2017depthcomp}
%     &     .436 &    .290 &    .155 &    79.4 &    94.7 &    98.6
%     &     .448 &    .297 &    .128 &    84.5 &    96.6 &    99.0
%     &*&*&*&*&*&*\\
% \hline
% Inpaint% \cite{iizuka2017globally}
%     &     .453 &    .300 &    .159 &    78.6 &    94.2 &    98.4
%     &     .430 &    .286 &    .121 &    86.2 &    97.0 &    99.5
%     &     .452 &    .299 &    .159 &    78.5 &    94.3 &    98.4\\
% Auto-encoder
%     &     .450 &    .297 &\bf .150 &    79.1 &    94.5 &    98.5
%     &\bf  .389 &\bf .266 &\bf .116 &    86.7 &\bf 98.2 &\bf 99.9
%     &     .450 &    .297 &\bf .149 &    79.2 &    94.5 &    98.5\\
% \hline
% Ours
%     & \bf .435 &\bf .290 &    .155 &\bf 79.5 &\bf 94.8 &\bf 98.6
%     &     .395 &    .274 &    .122 &\bf 86.8 &    98.1 &    99.8
%     &     .434 &    .289 &    .155 &    79.5 &    94.8 &    98.6\\
% \hline
% % Ours w/o mask
% %     &     .442 &    .301 &    .163 &    77.3 &\bf 95.1 &    98.4
% %     & \bf .384 &    .269 &    .120 &    86.2 &\bf 98.3 &    99.8
% %     &     .442 &    .301 &    .164 &    77.3 &\bf 95.1 &    98.4\\
% % Ours w/o norm
% %     &     .522 &    .358 &    .192 &    72.6 &    91.6 &    96.9
% %     &     .470 &    .330 &    .149 &    80.4 &    95.9 &    98.9
% %     &     .522 &    .357 &    .192 &    72.7 &    91.6 &    96.9\\
% % \hline
% \end{tabular}
% }%resizebox
% \end{center}
% \vspace{-1mm}
% \caption{Depth prediction~(with object removed) performance compare with other baselines on AI2-THOR testset (all examples in testset). Note that this testset contains several small objects, such that all pixels metric is greatly influenced by exterior pixels. It misleads to conclude that ours method does not improve compared to do nothing, when in fact it's bad.. % Autoencoder performs slightly better than ours in some metrics but it trashes at pixels outside the object mask.
% %Poisson and DepthComp only produce pixels within mask; that's why we report * in exterior columns where the values are equal to Do nothing. Our method outperforms baselines.
% %The last block is only for an ablation study of our network. We study the effect (or lack) of mask dropout (ours w/o mask) and normal loss (ours w/o normal). They make our network (ours) more reliable on both interior and exterior regions. 
% }
% % To better compare with these we make a special method to Autoencoder (C\&P AE) and ours (C\&P Ours) by copy and paste the exterior from the initial depth. Thus these C\&P methods have the same exterior, hence we clearly see the result of interior pixels.
% %\vspace{-1mm}
% %Metric from left to right: root mean square, absolute relative difference, $\delta <1.25$, $\delta <1.25^2$, and $\delta <1.25^3$.} %Note in left columns lower is better, while higher is better in right columns.}
% \label{table:supai2thor}
% \end{table*}








% \begin{table*}
% \begin{center}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
% \hline
%     & \multicolumn{6}{c||}{All Pixels}
%     & \multicolumn{6}{c||}{Interior}
%     & \multicolumn{6}{c|}{Exterior} \\
% \cline{2-19}
% Method
%     & rms & rel & norm & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & norm & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & norm & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
% \hline
% \multicolumn{19}{|c|}{Laina as depth prediction}\\
% \hline
% Do nothing
%     &     .714 & &   .306 &    51.5 &    80.3 &    92.9
%     &     .704 & &   .344 &    36.8 &    71.0 &    93.9
%     &     .714 & &   .305 &    51.9 &    80.5 &    92.9\\
% Inpaint %\cite{iizuka2017globally}
%     &     .728 & &   .311 &    51.2 &    79.6 &    91.9
%     &     .713 & &   .366 &    38.7 &    69.9 &    90.9
%     &     .729 & &   .310 &    51.4 &    79.8 &    91.9\\
% Poisson%\cite{perez2003poisson}
%     &     .714 & &   .305 &    51.6 &    80.3 &    92.8
%     &     .702 & &   .322 &    41.7 &    71.5 &    88.8
%     &     .714 & &   .305 &    51.9 &    80.5 &    92.9\\
% DepthComp%~\cite{atapour2017depthcomp}
%     & & & & & &
%     & & & & & &
%     & & & & & &\\
% Auto-encoder
%     &     .719 & &   .292 &    50.6 &    79.8 &    93.5
%     &     .666 & &   .374 &    38.4 &    67.0 &    94.8
%     &     .720 & &   .290 &    50.9 &    80.1 &    93.5\\
% \hline
% \multicolumn{19}{|c|}{Ours w/o mask as depth prediction}\\
% \hline
% Do nothing
%     &     .436 &    .155 &    14.19 &    79.5 &    94.7 &    98.5
%     &     .414 &    .118 &    26.99 &    85.9 &    97.5 &    99.7
%     & \bf .434 &    .155 &    13.93 &    79.6 &\bf 94.8 &\bf 98.6\\
% Inpaint% \cite{iizuka2017globally}
%     &     .453 &    .159 &    14.20 &    78.6 &    94.2 &    98.4
%     &     .430 &    .121 &    24.77 &    86.2 &    97.0 &    99.5
%     &     .452 &    .159 &    14.00 &    78.5 &    94.3 &    98.4\\
% Poisson% \cite{perez2003poisson}
%     &     .438 &    .156 &    14.27 &    79.2 &    94.5 &    98.4
%     &     .455 &    .133 &    28.01 &    83.7 &    95.1 &    97.5
%     %& \bf .434 &    .155 &    13.93 &\bf 79.6 &    94.8 &\bf 98.6\\
%     & * & * & * & * & * & * \\
% DepthComp%~\cite{atapour2017depthcomp}
%     &     .436 &    .155 &    14.25 &    79.4 &    94.7 &    98.6
%     &     .448 &    .128 &    29.20 &    84.5 &    96.6 &    99.0
%     %& \bf .434 &    .155 &    13.93 &    79.6 &\bf 94.8 &\bf 98.6\\
%     & * & * & * & * & * & * \\
% Autoencoder
%     &     .450 &\bf .150 &    14.08 &    79.1 &    94.5 &    98.5
%     & \bf .389 &\bf .116 &    26.96 &    86.7 &\bf 98.2 &\bf 99.9
%     &     .450 &\bf .149 &\bf 13.88 &    79.2 &    94.5 &    98.5\\
% \hline
% Ours
%     & \bf .435 &    .155 &\bf 14.05 &\bf 79.5 &\bf 94.8 &\bf 98.6
%     &     .395 &    .122 &\bf 24.23 &\bf 86.8 &    98.1 &    99.8
%     &     .434 &    .155 &    13.90 &    79.5 &    94.8 &    98.6\\
% \hline
% \end{tabular}
% }
% \end{center}
% \end{table*}




==> table-sup-eval.tex <==
% \begin{table*}
% \begin{center}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
% \hline
%     & \multicolumn{6}{c||}{All Pixels}
%     & \multicolumn{6}{c||}{Interior}
%     & \multicolumn{6}{c|}{Exterior} \\
% \cline{2-19}
% Method
%     & rms & rel & norm & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & norm & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & norm & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
% \hline
% Do nothing
%     &     .462 &&   .227 &    64.9 &    88.8 &    99.8
%     &     .480 &&    .211 &    50.8 &    87.0 &    99.6
%     &     .460 &&    .228 &    66.3 &    89.0 &    99.9\\
% Inpaint% \cite{iizuka2017globally}
%     &     .632 &&    .312 &    48.1 &    81.9 &    99.3
%     &     .633 &&    .294 &    39.7 &    90.3 &    100.0
%     &     .632 &&    .313 &    48.8 &    81.1 &    99.2\\
% Poisson% \cite{perez2003poisson}
%     &     .473 &&    .236 &    66.1 &    87.5 &    99.2
%     &     .394 &&    .178 &    73.4 &    93.8 &    99.8
%     &     .479 &&    .242 &    65.4 &    86.9 &    99.2\\
% DepthComp%~\cite{atapour2017depthcomp}
%     & && & & &
%     & && & & &
%     & && & & &\\
% Auto-encoder
%     &     .430 &&    .210 &    69.4 &    91.1 &\bf 99.9
%     &     .342 &&    .149 &    75.3 &    98.1 &    100.0
%     &     .438 &&    .216 &    68.9 &    90.5 &\bf 99.9\\
% \hline
% \end{tabular}
% }%resizebox
% \end{center}
% \end{table*}

\begin{table*}[!h]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
\hline
    & \multicolumn{6}{c||}{All Pixels}
    & \multicolumn{6}{c||}{Interior}
    & \multicolumn{6}{c|}{Exterior} \\
\cline{2-19}
Method
    & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
    & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
    & rms & mae & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
\hline
& \multicolumn{18}{c|}{Input depth map: Laina~\etal}\\
\hline
Do Nothing
    &     .462 &    .380 &    .227 &    64.9 &    88.8 &    99.8
    &     .480 &    .403 &    .211 &    50.8 &    87.0 &    99.6
    &     .460 &    .378 &    .228 &    66.3 &    89.0 &    99.9\\
Poisson% \cite{perez2003poisson}
    &     .473 &    .384 &    .236 &    66.1 &    87.5 &    99.2
    &     .394 &    .314 &    .178 &    73.4 &    93.8 &    99.8
    &     .479 &    .390 &    .242 &    65.4 &    86.9 &    99.2\\
DepthComp%~\cite{atapour2017depthcomp}
    &     .461 &    .378 &    .226 &    65.6 &    89.2 &    99.9
    &     .471 &    .382 &    .203 &    58.4 &    92.5 &    99.9
    &*&*&*&*&*&*\\
Inpaint% \cite{iizuka2017globally}
    &     .632 &    .529 &    .312 &    48.1 &    81.9 &    99.3
    &     .633 &    .545 &    .294 &    39.7 &    90.3 &    100.
    &     .632 &    .527 &    .313 &    48.8 &    81.1 &    99.2\\
Auto-encoder
    &     .430 &    .353 &    .210 &    69.4 &    91.1 &    99.9
    &     .342 &    .278 &    .149 &    75.3 &    98.1 &    100.
    &     .438 &    .360 &    .216 &    68.9 &    90.5 &    99.9\\
\hline
& \multicolumn{18}{c|}{Input depth map: Ours with empty object mask}\\
\hline
Do Nothing
    &     .447 &    .368 &    .207 &    67.0 &    90.6 &    99.6
    &     .600 &    .513 &    .267 &    35.8 &    67.6 &    97.0
    & \bf .430 &\bf .355 &    .201 &\bf 69.9 &    92.7 &    99.8\\
Poisson% \cite{perez2003poisson}
    &     .427 &    .352 &    .198 &    69.6 &    92.8 &    99.8
    &     .394 &    .320 &    .168 &    66.8 &    93.9 &    99.9
    %& \bf .430 &\bf .355 &    .201 &\bf 69.9 &    92.7 &    99.8\\
    &*&*&*&*&*&*\\
DepthComp%~\cite{atapour2017depthcomp}
    &     .438 &    .360 &    .203 &    68.0 &    91.6 &    99.7
    &     .513 &    .424 &    .225 &    47.9 &    79.7 &    98.8
    &*&*&*&*&*&*\\
Inpaint% \cite{iizuka2017globally}
    &     .538 &    .434 &    .258 &    60.2 &    86.4 &    98.9
    &     .526 &    .445 &    .235 &    52.3 &    92.6 &    99.8
    &     .539 &    .433 &    .260 &    60.9 &    85.9 &    98.8\\
Auto-encoder
    &     .431 &    .360 &\bf .192 &    66.0 &\bf 95.0 &\bf 100.
    &     .353 &    .290 &    .153 &    70.5 &    97.7 &    100.
    &     .437 &    .366 &\bf .196 &    65.5 &\bf 94.7 &\bf 100.\\
\hline
Ours
    & \bf .425 &\bf .349 &    .198 &\bf 70.6 &    93.0 &    99.8
    & \bf .310 &\bf .247 &\bf .133 &\bf 81.9 &\bf 99.6 &\bf 100.
    &     .435 &    .359 &    .204 &    69.5 &    92.4 &    99.8\\
\hline
\end{tabular}
}%resizebox


% \begin{table*}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|p{1.5cm}|c||c|c||c|c|c||c|c||c|c|c||c|c||c|c|c|}
% \hline
% Depth & Object Removal
%     & \multicolumn{5}{c||}{All Pixels}
%     & \multicolumn{5}{c||}{Interior}
%     & \multicolumn{5}{c|}{Exterior} \\
% \cline{3-17}
% Prediction & Method
%     & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
% \hline
% \multirow{5}{\linewidth}{Laina}
% & Do nothing
%     &     .462 &    .227 &    64.9 &    88.8 &    99.8
%     &     .480 &    .211 &    50.8 &    87.0 &    99.6
%     &     .460 &    .228 &    66.3 &    89.0 &    99.9\\
% & Inpaint \cite{iizuka2017globally}
%     &     .632 &    .312 &    48.1 &    81.9 &    99.3
%     &     .633 &    .294 &    39.7 &    90.3 &    100.0
%     &     .632 &    .313 &    48.8 &    81.1 &    99.2\\
% & Poisson \cite{perez2003poisson}
%     &     .473 &    .236 &    66.1 &    87.5 &    99.2
%     &     .394 &    .178 &    73.4 &    93.8 &    99.8
%     &     .479 &    .242 &    65.4 &    86.9 &    99.2\\
% & DepthComp~\cite{atapour2017depthcomp}
%     & & & & &
%     & & & & &
%     & & & & &\\
% & Auto-encoder
%     &     .430 &    .210 &    69.4 &    91.1 &\bf 99.9
%     &     .342 &    .149 &    75.3 &    98.1 &    100.0
%     &     .438 &    .216 &    68.9 &    90.5 &\bf 99.9\\
% \hline
% N/A & Ours
%     & \bf .425 &\bf .198 &\bf 70.6 &\bf 93.0 &    99.8
%     & \bf .310 &\bf .133 &\bf 81.9 &\bf 99.6 &\bf 100.0
%     & \bf .435 &\bf .204 &\bf 69.5 &\bf 92.4 &    99.8\\
% \hline
% \end{tabular}
% }%resizebox
% \begin{center}

%\resizebox{0.99\linewidth}{!}{
% \begin{tabular}{|c||c|c||c|c|c||c|c||c|c|c|}
% \hline
%     & \multicolumn{5}{|c||}{Interior}
%     & \multicolumn{5}{c|}{Exterior} \\
% \hline
% Method
%     & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$
%     & rms & rel & $\delta_1$ & $\delta_2$ & $\delta_3$  \\
% \hline
% Do nothing
%     & 0.492     & 0.216     & 48.2      & 86.1      & 99.6
%     & 0.462     & 0.227     & 64.9      & 88.8      &  99.8\\
% Poisson \cite{perez2003poisson}
%     & 0.366     & 0.157     & 70.4      & 96.9      & \bf 100.0
%     & 0.453     & 0.222     & 66.6      & 89.6      & 99.8\\
% Inpaint \cite{iizuka2017globally}
%     & 0.506     & 0.232     & 57.2      & 95.2      & \bf 100.0
%     & 0.516     & 0.245     & 63.0      & 87.7      & 99.8\\
% DepthComp~\cite{atapour2017depthcomp}
%     & 0.467     & 0.191     & 62.8      & 93.3      & 99.9
%     & 0.461     & 0.226     & 65.6      & 89.3      & \textbf{99.9}\\
% Auto-encoder
%     & 0.344     & 0.141     & 78.1      & 98.4      & \bf 100.0
%     & 0.430     & 0.210     & 69.4      & 91.2      & \textbf{99.9}\\
% Ours
%     & \bf 0.310 & \bf 0.132 & \bf 81.7  & \bf 99.5  & \bf 100.0
%     & \bf 0.426 & \bf 0.199 & \bf 70.4  & \bf 93.0  & 99.8\\
% \hline
% \end{tabular}
%}%resizebox
\end{center}
\vspace{-1mm}
\caption{Depth prediction~(with object removed) performance compared with other baselines on our collected evaluation dataset. We evaluate average pixel performance on: all image pixels, middle: pixels inside the object mask~(interior) and pixels outside the object mask~(exterior). Even though ours with empty object mask is better as a input depth map for those baselines, auto-encoder using Laina \etal as the input depth map is better than using ours in some metrics. However, our method is the best in most metrics.
% We evaluate average pixel performance on: all image pixels, middle: pixels inside the object mask~(interior) and pixels outside the object mask~(exterior).  Our method outperforms baselines by a substantial margin.
}
\vspace{-3mm}
%Metric from left to right: root mean square, absolute relative difference, $\delta <1.25$, $\delta <1.25^2$, and $\delta <1.25^3$.} %Note in left columns lower is better, while higher is better in right columns.}
\label{table:supeval}
\end{table*}
